What if AI systems weren't chatbots?

The rapid convergence of artificial intelligence (AI) toward conversational chatbot interfaces marks a critical moment for the industry. This paper argues that the chatbot paradigm is not a neutral interface choice, but a dominant sociotechnical configuration whose widespread adoption reshapes social, economic, legal, and environmental systems. We examine how treating AI primarily as conversational assistants has extensive structural downsides. We show how chatbot-based systems often fail to adequately meet user needs, particularly in complex or high-stakes contexts, while projecting confidence and authority. We further analyze how the normalization of chatbot-mediated interaction alters patterns of work, learning, and decision-making, contributing to deskilling, homogenization of knowledge, and shifting expectations of expertise. Finally, we examine broader societal effects, including labor displacement, concentration of economic power, and increased environmental costs driven by sustained investment in large-scale chatbot infrastructures. While acknowledging legitimate benefits, we argue that the current trajectory of AI development reflects specific value choices that prioritize conversational generality over domain specificity, accountability, and long-term social sustainability. We conclude by outlining alternative directions for AI development and governance that move beyond one-size-fits-all chatbots, emphasizing pluralistic system design, task-specific tools, and institutional safeguards to mitigate social and economic harm.

==> Makefile <==
TEX = main
BIB = sample-base

.PHONY: $(TEX).pdf clean

$(TEX).pdf: $(TEX).tex $(BIB).bib acmart.cls
	rm -f $(TEX).pdf
	pdflatex -interaction=nonstopmode $(TEX)
	bibtex $(TEX)
	pdflatex -interaction=nonstopmode $(TEX)
	pdflatex -interaction=nonstopmode $(TEX)

clean:
	rm -f $(TEX).aux $(TEX).bbl $(TEX).blg $(TEX).log $(TEX).out $(TEX).toc \
	      $(TEX).lof $(TEX).lot $(TEX).fls $(TEX).fdb_latexmk $(TEX).synctex.gz \
	      $(TEX).nav $(TEX).snm $(TEX).vrb $(TEX).xdv $(TEX).bcf $(TEX).run.xml \
	      $(TEX).cpt $(TEX).glo $(TEX).ist $(TEX).acn $(TEX).acr $(TEX).alg \
				comment.cut

